ENCORE: Ensemble Learning using Convolution Neural Machine Translation for Automatic Program Repair

Automated generate-and-validate (G&V) program repair techniques typically rely on hard-coded rules, only fix bugs following specific patterns, and are hard to adapt to different programming languages. We propose ENCORE, a new G&V technique, which uses ensemble learning on convolutional neural machine translation (NMT) models to automatically fix bugs in multiple programming languages. We take advantage of the randomness in hyper-parameter tuning to build multiple models that fix different bugs and combine them using ensemble learning. This new convolutional NMT approach outperforms the standard long short-term memory (LSTM) approach used in previous work, as it better captures both local and long-distance connections between tokens. Our evaluation on two popular benchmarks, Defects4J and QuixBugs, shows that ENCORE fixed 42 bugs, including 16 that have not been fixed by existing techniques. In addition, ENCORE is the first G&V repair technique to be applied to four popular programming languages (Java, C++, Python, and JavaScript), fixing a total of 67 bugs across five benchmarks.

==> Makefile <==
all: *.tex
	pdflatex paper
	bibtex paper
	pdflatex paper
	pdflatex paper
	@echo '*******************************************************************************'
	@echo '***                  Did you spell-check the paper?                         ***'
	@echo '***      Did you make sure the paper compiles before you commit?            ***'
	@echo '*******************************************************************************'

purge:
	rm -f   *.aux \
                *.bbl \
                *.blg \
                *.dvi \
                *.log \
                *.toc \
                paper.ps \
		paper.pdf

clean:
	rm -f   *.aux \
                *.bbl \
                *.blg \
                *.dvi \
                *.log \
                *.toc \
                *.out \
                paper.ps



==> tab/tuned.tex <==
\begin{table}[t]
\centering

\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|}
	\hline
	\textbf{Parameters} & \textbf{\tool1} & \textbf{\tool2} & \textbf{\tool3} & \textbf{\tool4} & \textbf{\tool5}\\ \hline
	Enc. and dec. Input Embedding dim. & 232 & 398 & 54 & 139 & 430 \\ \hline
	Dec. output embedding dim. & 472 & 259 & 494 & 187 & 212 \\ \hline
	Enc. and dec. layers dim. & (640,3) * 2 & (640,4) * 2 & (512,9) * 3 & (640,7) * 6 & (384,10) * 10 \\ \hline
	Dropout & 0.07 & 0.15 & 0.08 & 0.17 & 0.18 \\ \hline
	Clip Normalization & 0.48 & 0.72 & 0.90 & 0.63 & 0.81 \\ \hline
	Optimizer & nag & sgd & sgd & nag & nag \\ \hline
	Cross Entropy Criterion & smoothed &  smoothed &  default & default & default \\ \hline
	Learning Rate & 0.78 & 0.41 & 0.43 & 0.88 & 0.58 \\ \hline
	Momentum & 0.80 & 0.74 & 0.73 & 0.78 & 0.83 \\ \hline
	
	\end{tabular}
	}
	\label{tab:tuning_info}
	\caption{General information from our dataset.}
\end{table}

